Detectability of satellites around directly imaged exoplanets and brown dwarfs

Satellites around substellar companions are a heterogeneous class of objects with a variety of different formation histories. Focusing on potentially detectable satellites around exoplanets and brown dwarfs, we might expect to find objects belonging to two main populations: planet-like satellites similar to Titan or the Galileian Satellites - likely formed within the scope of core accretion; and binary-like objects, formed within different scenarios, such as disk instability. The properties of these potential satellites would be very different from each other. Additionally, we expect that their characterization would provide insightful information about the history of the system. This is particularly important for planets/brown dwarfs discovered via direct imaging (DI) with ambiguous origins. In this paper, we review different techniques, applied to DI planets/brown dwarfs, that can be used to discover such satellites. This was achieved by simulating a population of satellites around the exoplanet $\beta$ Pic b, which served as a test case. For each simulated satellite, the amplitude of DI, radial velocity, transit and astrometric signals, with respect to the planet, were retrieved and compared with the detection limits of current and future instruments. Furthermore, we compiled a list of 38 substellar companions discovered via DI to give a preliminary estimate on the probability of finding satellites extracted from the two populations mentioned above, with different techniques. This simplified approach shows that detection of planet-like satellites, though not strictly impossible, is very improbable. On the other hand, detection of binary-like satellites is within the capabilities of current instrumentation.

==> referee2.tex <==
TO THE EDITOR

Dear Bella,

Here below you can find our answers to this second referee report.
I want to express my disappointment for the behaviour of the referee that, even this second time, needed two months to revise the paper. Moreover, some of the major comments are, in my opinion, really marginal (such as first part of major comment 3), some are spurious (such as major comment 13 and minor comment 1) asking to give reference for equations that are widely known to most people since mid-school, and others ask for implementing something that is already in the paper (see major comment 13 about the orbital stability). The referee is also asking (for the second time) to change au in A.U. which is against the directive given by the IAU (see minor comment 8).
It would be really much appreciated if this time at least the referee could carefully and quickly read the manuscript and check twice before adding further useless comments.








Assistant editor comments;
Please provide some information about why a new author was added to the paper - my software notes this as unusual activity and I have to provide a justification.
The abstract is now 300 words, well over the 250 word guideline to authors. Please re-write the abstract to fit.
The text & number labels on some of your figures are too small. Please ensure that they are at least as big as the body text wherever possible. Also consider the legibility of sub- and superscript text and numbers. Figure 3 would benefit by changing black text on dark blue to white, or another light colour.
Your last reference is not in alphabetical order.

Answer: PhD student Shrishmoy Ray was added to proof read the paper as language editing was requested in the first revision.
The abstract now is below 250 words.
Plots were changed following the advices and requests of the assistant editor.
Reference fixed.




TO THE REFEREE

Reviewer's Comments:
Reviewer: 1

Comments to the Author
Sincere thanks to the authors for a very substantial revision to the manuscript from its previous version.  It is clear that the authors have undertaken a lot of extra work to improve the paper's content and conclusions, and their extra work is to be commended.

Thank you also to the authors for having taken up many of the suggestions in the first referee report, it is very clear that several of these have been adopted, and in my opinion, have increased the clarity of the paper.  

I am afraid I still have substantial reservations about the
conclusions of this paper, and would suggest major modification of the
manuscript before it is suitable for publication in MNRAS.  Some of
the concerns are left over from the previous version, and some are
new.  

1. Even the second time around, it took me a second reading before it became clear that all the different techniques being explored for the detection of the satellite were referenced to the planet, rather than to the parent star.  I would urge the authors to clarify this point and make it clear from the very outset that what is being explored is direct imaging, RV, transits and astrometry relative to the planet.

Answer: We further specified this in the introduction (pg 2, LHS, second-last paragraph of sec 1) and in Section 3 (pg 3, LHS, last paragraph of sec 3) 

2. I felt that a large part of the manuscript's conclusions are to be
drawn from Tables 2 and 3. Table 2 appears to suggest that if a planet
has a satellite (i.e. f = 1) that is of the "binary" type, then the
detection probability is very close to 1 for astrometry and RV, and
also above 97\% for direct imaging, with a 43\% probability for
transits.  However, looking at Table A1 in the appendix, I fail to
find any numbers for the probabilities that are above one-third, let
alone close to 1! There must be some simple explanation for this
discrepancy, but I have missed it completely.  Even for f=0.14, the
numbers are much higher than any of the probabilities in Table A1.
Can the authors please clarify what is meant in Table 2.

Answer: The probabilities P_tot reported in Table 2 are for the detection of at least one satellite by observation of the whole sample of 38 planets. This is different from the probability p_i of detecting a satellite around each planet in the sample (reported in Tables A1 and A2). 
We added this comment in Section 4.4 (pg 9, RHS, second paragraph of sec 4.4)

3. Figure 1 shows the parameter space accessible to direct imaging
detection of a satellite around beta-Pic-b.  It is the only figure
where both x and y axis are linear, whereas all other techniques show
the mass range and separation in log units. It is a sensible choice, given how small
the accessible parameter space is. However, it would be good to point
this out explicitly, or use log scaling to highlight how small the
parameter space is.  
Also, it took me a long time to understand that
the contrast was meant to be w.r.t. the parent star, not the
planet. Can you please clarify this in the text and the figure
caption.   Given this plot, which shows that essentially the only
satellite that is observable is almost equal in mass to beta Pic b,
(11 M_J vs 13.8 M_J, a mass ratio or q_s = 0.8, I don't understand why
Table A1 lists the q_min for imaging as 0.5882, and the q_median as
0.7862, both below the detection limit.  Like I said earlier, I am not
sure I understand the analysis presented in Section 4 at all!

Answer: We added the comment of the referee about linear scales for DI (pg 3, RHS, first paragraph of sec 3.1) and also stressed in the text that the contrast is wrt the star and not the planet (pg 3, RHS, first paragraph of sec 3.1 and caption of fig 1).
About the contrast curves shown in Fig 1 and the results of Table A1, the two analysis where obtained following different procedure. Especially the analysis presented in Sec 4.3.1 is a rough estimate of the contrast to be considered as order of magnitude more than a precise result. We added a comment in the last paragraph of section 4.3.1 (pg 9, LHS).

4. In section 3.1, you use a magnitude range of 2 Mags (fainter) relative to the planet itself, which seems reasonable for DI, and subsequently convert it to the mass of the satellite.  Yet, in Section 4.3.1, you derive limits on the K magnitude of the putative satellite by a very different method, clearly coming up with a very different range in magnitude, not only for Beta Pic b, but for all planets. I am not sure I agree with the values used in Section 4.3.1 - In the absence of contrast issues from star or planet, you are claiming that the K band limiting apparent magnitude is 19.6+4.2 = 23.8.  What exposure time is assumed to achieve this limiting magnitude?

Answer: The contrast achievable in DI should depend on the separation between the satellite and the planet, as well as on the magnitude of the planet itself and on the separation from the star. Since the limiting contrast is defined as that for which a SNR=5 is obtained, the limiting contrast depends on noise; the approach we follow in Section 4.3.1 is to consider various sources of noise, that are summed in quadrature. 
The exposure time is 3600 sec=1 hr.
We added the sentence “The following calculations are obtained assuming good-quality observations of 1 hr taken from a 8-meter size telescope during meridian passage.” at the end of the first paragraph of sec 4.3.1



5. While you quote formulae for all the different terms contributing to the limiting contrast due to the parent star, you do not provide a
simple plot of this contrast w.r.t. d (the star-planet
separation). May I suggest that you add such a plot, so that it is
easy to visualize what contrast limits you are using. Are these values consistent with those used in Sec 3.1 for the Beta Pic b simulation?
If not, why not?

Answer: We added a plot showing the limiting contrast for satellite detection due to the planet background as a function of planet-satellite separation provided by the formula used in the text. Note that this sums in quadrature with other sources of background as given by eq. (7), so that the actual limit may be brighter depending on the particular planet we consider.

6. For the planet contrast, if I stick in x = 1000 mas in your formula at
the bottom of page 9, LHS, I get c_p = Delta_K_P - 2.5*(2.9*10^9)  -
clearly this is incorrect, suggesting a problem with units.   Is x 
supposed to be in arc seconds,
perhaps?  I then get a contrast of 1.68 mag relative to the planet at
1 arcsec - which is a modest, conservative estimate.  However, your
Table 1 does not include the H or K magnitudes of the planets, so I
cannot compute this part - can you please add the planet magnitudes to
Table 1.

Answer: We revised this formula, that was too optimistic at very short separations; results are however very similar because there are other limitations to the contrast to be considered (stellar and sky background). Anyhow, the formula can only be used up to separation of 220 mas. At this large separation the planet background is negligible with respect to the sky background. 
We added the planet K-band magnitude used in this paper in Table 1. Note that they are derived with the formulas considered in this paper - starting form masses and ages - and they are not the observed values.

7. Is there a certain telescope size assumed (in terms
of the diffraction limited PSF width)? Later on, you generalise your
conclusions to ELT, JWST and other telescopes - are you sure the right
scaling has been included before these conclusions are drawn?

Answer: The calculation are obtained wrt a 8-meters size telescope. We added this comment to Section 4.3.1 (pg 8, RHS, first paragraph of sec 4.3.1)

8. Section 4.3.2 talks of RV limits, and has a scaling law for the
detectable amplitude of the RV signal from the satellite as
0.1*10^(0.2*(K_P-13.5)).  I cannot see how this works, as when the
planet gets fainter the RV limits get smaller. e.g. K_P = 18.5 gives
RV limit of 0.110 km/s, while K_P = 23.5 gives 0.012 km/s - so I
understand this as saying that any satellite generating a 12 m/s
signal around a 23.5 mag planet is detectable!

Answer: The referee used the formula 0.110^(0.2*(K_P-13.5)) while we meant 0.1*10^(0.2*(K_P-13.5)). The formula was written correctly (there is a space between 0.1 and 10) but could easily be misunderstood. We wrote again as 0.1\times 10^(0.2*(K_P-13.5)) to be more clear.

9. Section 3.2 discusses the RV technique for satellite detection in the
context of Beta Pic b. The planet has a K mag of 13.8, and the main
source of uncertainty in the RV determination is the limited photon
flux, particularly if high-resolution spectrograph such as CRIRES+ is
to be used.  Are you sure you can achieve the RV accuracy of 100 m/s,
even assuming that you are only photon noise limited? What spectrum
did you assume for the planet flux? (these issues were pointed out
before, but haven't been addressed adequately).  I have had a detailed read of 
Vigan et al. 2018, and they do not quote the accuracy of 85 m/s within
1 hour of observation for the *PLANET* RV, contrary to what is stated
in Lines 9 through13 on page 5.

Answer: Rather than referring to Vigan et al. (2018), we presented new arguments about the accuracy of RV for planets/BDs around stars. Using the ETC (https://etc.eso.org/observing/etc/crires), the expected SNR in the H-band on beta Pic b with CRIRES is about 40 per pixel in 1 hr (with 6x600 sec DITs) using the natural guide star AO on the primary. However, in this mode the dominant source of noise for beta Pic b should be the stellar background, that is not included in the SNR estimate. The stellar background is efficiently removed using HiRISE, that is however less transmitting than the direct train to CRIRES by a factor of about 15 - though this is partly offset by the ~3 times higher Strehl provided by SPHERE with respect to MACAO. We simulate this lower efficiency considering an object with H=15.5, rather than H=13.8. The SNR per pixel in this condition is about 10. To transform this into an error in RV, we may consider the observations of TW Hya made by Figueira et al. (2010, A&A 511, A55) where an internal accuracy of 6 m/s was obtained from spectra with SNR~230 (this value has been traced back using the ETC, considering the stellar magnitude, the observing mode, DIT and number of exposures). Ignoring the much larger wavelength coverage of CRIRES+ with respect to CRIRES, the expected RV accuracy of a SNR=10 observation for a late M object should then be ~140 m/s, but it can well be a factor of 1.5 better considering the much wider spectral range, in agreement with our assertion of an error of 85 m/s in 1 hr observation on beta Pic b.
We added this derivation in Section 3.4 
We note that when considering the whole sample considered in Table 1, the gain using best performing AO but lower transmission of HiRISE with respect to MACAO should be considered object-by-object. We added a sentence about this at the end of Section 4.3.2

10. Please also explain what Section 3.2 adds to our knowledge that is not
already presented in Vigan et al. 2018, or Vanderburg et al. 2018.

Answer: The argument about the precision of RV determinations for planets/BDs around stars is completely new.

11. Even if the assumptions made about RV accuracy were to be true, it is
clear that roughly 100 hours of observations would be needed to get
enough RV data to look for a signature of a satellite, making this
proposed method prohibitive in terms of exposure time.

Answer:  The referee is completely right. Indeed, we already mention this in the paper (pg 5, LHS, last paragraph of sec 3.2 and in Sec 4.4). To further stress the concept, we added some more reflections in Sec 4.4 (pg 10, LHS, third paragraph of sec 4.4).

12. Section 3.3 deals with the transit method.  The double valued nature
of the plot in Figure 3, where the filling in of the transit by the
self-luminosity of the satellite means that a large mass ambiguity
will exist. This needs to be discussed in the paper.  Moreover, the
20\% flux uncertainty in the photometry that they assume (following
Biller et al. 2021)  is for each AO assisted observation, and is not
automatically the limit for the flux reduction during the transit.
Given the uncertainty in the AO PSF, it would be extremely difficult
to detect a transit via monitoring of the planet flux. The author's
own data from DH Tau B should showcase the uncertainty.

Answer:  The referee is completely right. We have already added mention to the limit related to AO assisted instruments. We added further comments on the limitations of this technique (pg 6, end of the first paragraph on the LHS column) 



13. All the different methods limit themselves to round orbits, and do not
look at the dynamical stability of the orbits they explore.  I think
this is a severe limitation, as we know that any satellite that will
be observed will likely be in a dynamically stable configuration.  If
equations, such as that for the Hill radius or the Roche limit, are
not derived by the authors, but are simply copied from a text or
paper, it is imperative that the authors provide the reference in each
case.  This is an issue throughout the manuscript.

Answer: Following the suggestion of the previous report we actually included the stability for round, prograde orbits (see second paragraph of section 3). We do not think that including eccentricity to the analysis will enrich significantly the paper giving the preliminary estimates given.
For what regard both citations for the Hill radius and Roche limit equations, the derivation goes back to the first half of 19th century and it is really hard to find the original work from  Édouard Roche (or even another paper with citations to these equations).
If the referee could help us suggesting a reference we would be extremely grateful.


14. Section 3.4 deals with astrometry. Although the GRAVITY instrument is
superb at providing astrometry, the quoted paper mentions 10th
magnitude (bright) targets.  Sadly, very few directly imaged planets
are 10th magnitude.  Thus, given that the full orbit is rarely well
determined (Beta Pic being the exception), and given the faintness of
the planet, the stated sub-mas accuracy is not achievable, either with
current instrumentation, or any time in the near future.

Answer: The astrometric measure we consider here is the relative position of the planet with respect to the star; the presence of the satellite is deduced from the residuals of the planet motion wrt to a simple Keplerian around the star. So the target brighter than 10th mag that we have to consider here is the star. Actually astrometric measures of planet positions with an accuracy <0.1 mas have been already obtained for e.g. beta Pic b and c (Lacour et al. 2021, A&A, 654, L2); this is the reason of the limit at 0.3 mas we consider in Section 4.3.4.
If the planet orbit is much longer than the satellite one, then detection of the wobble due to the satellite does not require to follow the full planet orbit, but only the full satellite orbit (this is the reason we set an upper limit of 20 yr to the period of orbits detectable through astrometric signal with Gravity). In principle, we cannot tell from this data if the wobbling is due to a satellite around the planet or an additional planet around the star; however, absolute astrometry from Gaia may solve this ambiguity in the near future.
Some sentences explaining this were added in Section 3.4.

15. Page 8 of 21, LHS, lines 39-45: the sigma is stated, but not the mean
for the a value (or rather log a value).  Please make sure that you
provide enough information for someone reading your paper to be able
to reproduce your analysis.

Answer: We added the expression for the mean in the text (LHS, pg 8 second paragraph of section 4.2). For the mean value, instead, we used the expression $a=\log_{10}(0.45*(M_P/30.0)^{0.77})$, where $M_P$ is the mass of the planet expressed in Jupiter masses. This formula was obtained by assuming that the peak of the satellite formation is close to the ice-line around very young planets. This position was then derived by fitting the isochrones at 1 Myr from \citet{Baraffe2003}.

16. Page 8 of 21, RHS, lines 14-16: talks of a log-normal surface density
of binary companions.  What is the surface?  I don't understand at all
what the authors are trying to say here. 

Answer: This was a wrong expression by ourselves. We then replaced the term "surface density" with "semi-major axis distribution"





-----------

Minor issues:


1. Hill radius: the equation could usefully be re-stated here (as are
several others), and the reference provided.

Answer: we decided to remove the equation for Hill radius since the referee was asking for a reference, if explicitly written in the text. Now, this relation is widely used and known by the entire scientific community. Nevertheless, we couldn't find any reference for it, probably because it was derived roughly 200 years ago.




2.Introduction: it is stated that the DI method allows parameters to be
determined that cannot be quantified by other methods, but the
examples given could also be derived from transit measurements.
Please rephrase the discussion of the merits of DI.

Answer: the text quotes 
"In the past decade, the direct imaging (DI) technique has proven to be an inestimable method to investigate planetary systems. In fact, even if the indirect methods such as radial velocities (RV) and transits are more prolific in terms of the number of detections, substellar companions detected via direct imaging reveal a plethora of information on the object. "
There is no mention to the fact that DI is the only method to retrieve such parameters. We added a "simultanuesly" hoping that now the merits of DI are clearer.




3. Page 2 (of 21), RHS, lines 51-54: The text is more like a conclusion,
and is out-of-place in this section. Please consider moving it to the
conclusions.

Answer: we removed the sentence. 





4. Page 3 (of 21), LHS, lines 21-24: only 3 objects are cited previously,
of which two are exceptions, so don't really see how this can be seen
as confirmation of the hypothesis.

Answer: we are not referring only to the three candidates but also to the few brown dwarfs pairs that were detected in the previous years.
However, since the sentence is not of extreme importance to the purposes of the paper, we removed it


5. Table 1 shows the parameters for HR8799 planets as from a paper that
is "in prep" - while I appreciate there may be updates to the
parameters, surely there are other references for HR8799 that could
equally well be used, rather than await Zurlo et al. 2022! Please amend.

Answer: the paper is now submitted and will probably be accepted by the time we will receeve the next report. We would like to keep this parameters in the analysis since they are more updated and precise. 



6.Section 3 (the intro, prior to Sec 3.1) talks about using masses in
the range 0.001 to 1 M_P, with log-steps of 0.01 M_Jup. Can you please
justify both the choice of range and step-size.  The same applies for
the step size of the semi-major axis.

Answer: there is no particular reason for the choice of the step-size if not for visual purposes in the plots (which we do not think it is worth mentioning in the paper).
For what regards the range of masses, the lower limit takes into account sub-earth-like satellites up to binary objects (we added this comment to the text).
The semi-major axis range is already justified in the text (tidal disruption for the lower limit and dynamical stability for the upper limit).



7. Page 4 (of 21), LHS, lines 40-41: Please state which ELT instrument is
assumed in the claim that ELT will be able to explore nearby stars of
any age range for the presence of planets in reflected light.  Also,
please remove the following speculative sentence, as it is not borne
out by the detailed analysis presented in this manuscript.

Answer: we removed the sentence


8. Note also, A.U. needs to be capitalised, as it stands for Astronomical Unit

Answer: the IAU official site states that astronomical units must be referred to as au in scientific papers.
Here you can find the link to the webpage
https://www.iau.org/publications/proceedings_rules/units/#:~:text=The%20symbol%20for%20the%20astronomical,symbol%20inconvenient%20for%20general%20use
